Large-Scale Privacy-Preserving Network Embedding against Private Link Inference Attacks

Network embedding represents network nodes by a low-dimensional informative vector. While it is generally effective for various downstream tasks, it may leak some private information of networks, such as hidden private links. In this work, we address a novel problem of privacy-preserving network embedding against private link inference attacks. Basically, we propose to perturb the original network by adding or removing links, and expect the embedding generated on the perturbed network can leak little information about private links but hold high utility for various downstream tasks. Towards this goal, we first propose general measurements to quantify privacy gain and utility loss incurred by candidate network perturbations; we then design a PPNE framework to identify the optimal perturbation solution with the best privacy-utility trade-off in an iterative way. Furthermore, we propose many techniques to accelerate PPNE and ensure its scalability. For instance, as the skip-gram embedding methods including DeepWalk and LINE can be seen as matrix factorization with closed form embedding results, we devise efficient privacy gain and utility loss approximation methods to avoid the repetitive time-consuming embedding training for every candidate network perturbation in each iteration. Experiments on real-life network datasets (with up to millions of nodes) verify that PPNE outperforms baselines by sacrificing less utility and obtaining higher privacy protection.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> introduction.tex <==
\section{Introduction}
Network data such as citation networks, social networks, communication networks and so on, is ubiquitous in human life. In order to better utilize these data, more and more data holders are willing to share them with others to mining the hidden value. {\color{red}(references)} However, it has been proved that directly publishing the informative network data will lead to severe privacy leakage problem. {\color{red}(references)} Therefore, how to design an effective privacy-preserving data publishing method to reduce the privacy leakage risk when publishing network data is an urgent problem to be solved. 

Recently, network embedding technique is prosperous, which is a low-dimensional representation method for network data. {\color{red}(references)} With this technique, each node is represented by a low-dimensional vector, and the network information is embedded in these vectors, which then can be used to deal with the downstream tasks like node classification{\color{red}(references)}, clustering{\color{red}(references)} and link prediction{\color{red}(references)}. Meanwhile, to some extent, network embedding can be regarded as a privacy-preserving representation of the network data, due to its simplicity and uninterpretability. Can we just publish the network embedding instead of the network data to bring down the privacy leakage risk?

Unfortunately, the answer is no. It looks like users’ attributes and relationships are hidden by publishing low-dimensional network embedding, however, actually, users’ private information is still vulnerable to attacks, because existing network embedding techniques do not take the privacy issues into account when designing. Once the attackers obtain the released network embedding, it’s a piece of cake for them to infer the private information of users by training a machine learning attack model. For instance, it’s free for Facebook users to set their friend list inaccessible to anyone else except herself. We call these users with high privacy awareness \textit{private nodes}, and the relationships between them, called \textit{private links}, are expected to be hidden. However, attackers can easily infer these private links with a high accuracy when the network embedding is released, which means users’ private information is leaked in the process of data release.

Existing privacy-preserving data publishing methods cannot preserve users' private links against inference attack when network embedding is released. Firstly, most of previous studies concentrate on the tabular data {\color{red}(references)} which is totally different from the network data. Secondly, the studies which focus on network data usually publish the entire network, rarely considering about the network embedding publishing problem {\color{red}(references)}. Recently, adversarial attack techniques on network {\color{red}(references)} have provided some ideas. From the perspective of adversarial machine learning, these attacks aim to reduce the performance of the downstream tasks by adversarially manipulating the network structure or node attributes. Specifically, we may use this idea to defend against the malicious data recipients who want to infer users' private links. However, directly employing the adversarial attack techniques will incur large utility loss, i.e., they assume that each link in the network has the same utility.

In order to preserve users’ private links against inference attack, we would like to purposefully obscure the network data by manipulating its structure via adversarial learning before the release of the network embedding. However, obscuring always leads to a data utility degradation. Actually, it is a privacy-utility tradeoff problem, which aims to use the minimum utility loss of network embedding to trade the maximum privacy protection against private links inference attack. In this work, we aim to tackle a novel \textbf{privacy-preserving network embedding publishing problem}: how to design an obscuring mechanism for the network data to preserve the private links, meanwhile retaining the data utility for the downstream tasks when the network embedding based on the obscured network data is published?

We have the following difficulties to solve the problem.\textbf{ Firstly}, how to quantify the privacy leakage of private links caused by network embedding publishing? As far as we know, this work is the first work to study the privacy leakage of private links resulted from network embedding publishing. \textbf{Secondly}, how to measure and control the utility distortion of network embedding when obscuring? \textbf{Thirdly}, the optimization of the privacy-utility tradeoff problem is not trivial. Even though we find a method to properly quantify the privacy leakage and the utility loss appropriately, we need to design a mechanism to approach the optimal privacy-utility tradeoff.

This work overcomes the above challenges and our key contributions are as follows:
\begin{itemize}
	\item We quantify the privacy leakage of private links when publishing network embedding, and formulate the privacy-preserving network embedding problem, which aims to minimize the privacy leakage under a guaranteed data utility loss by obscuring the network structure deliberately.
	\item We quantify the network embedding utility loss caused by obscuring and propose a framework called \textit{PPNE}, which obscures the network structure via adversarial learning. To the best of our knowledge, this is the first work to use the adversarial attack techniques to protect users' private information on network data.
	\item We extensively evaluate our method with three real-life datasets, two attacker prior knowledge scenarios and two utility applications. The results show that \textit{PPNE} outperforms the state-of-art baselines, which means that our method achieves the best privacy-utility tradeoff.
\end{itemize}

==> preliminary.tex <==
\section{Preliminary on Network Embedding}

%In this section, we first introduce key prior works on network embedding, which are closely related to our research. Then, we formulate our research problem of \textit{Privacy-Preserving Network Embedding Publishing against Link Prediction Attacks}.
%This section introduces the preliminary knowledge of network embedding and formulate the problem to investigate in this paper.

%Table~\ref{tab:freq} summaries the math notations used throughout the text.
%
%\begin{table}[t!]
%	\caption{Math notations.}
%	\label{tab:freq}
%	\begin{tabular}{cl}
%		\toprule
%		Notation&Description\\
%		\midrule
%		$A$ & The original network.\\
%		$A'$ & The manipulated network for privacy preserving.\\
%		$\mathscr{P}$ & The set of private node pairs in $A$.\\
%		$\mathscr{P}_{pos}$ & Positive user pairs indicating existence of links.\\
%        $\mathscr{P}_{neg}$ & Negative user pairs indicating absence of links.\\
%        $X$ & Network embedding on original network.\\
%        $X'$ & Network embedding on manipulated network.\\
%        $Y$ & Context embedding learned together with $X$.\\
%        $M$ & The matrix factorized in DeepWalk and LINE. \\
%        $PL(X;\mathscr{P})$ & Privacy leakage when publishing $X$ given $\mathscr{P}$.\\
%        $\mathcal{L} (X;A)$ & The embedding quality loss of $X$ given $A$.\\
%		\bottomrule
%	\end{tabular}
%\end{table}

%\subsection{Network Embedding}
In this work, we focus on an undirected network, which is defined as $G=\left( V, E \right) $, where $V=\{v_i\}$ is the set of nodes and $E$ is the set of undirected edges between the nodes. Let $A\in \{0,1\}^{|V| \times |V|}$ denotes the adjacency matrix of $G$, and $a_{ij}=1$ when there is an edge between $v_i$ and $v_j$ and 0 otherwise. We can use $G$ and $A$ interchangeably to denote a network. The goal of the network embedding is to learn a function that maps all nodes in $V$ to low-dimensional representations $X \in \mathbb{R}^{\left| V \right| \times d}$, $d \ll \left| V \right|$, where the $i$-th row of $X$ is the $d$-dimensional representation of node $v_i$. The representations can be the inputs of machine learning models for various downstream tasks, such as node classification and clustering.

\subsection{Network Embedding Methods}
In this work, we mainly consider two representative network embedding  methods, DeepWalk~\cite{perozzi2014deepwalk} and LINE~\cite{tang2015line}. %Note that our studied problem and proposed method are not limited to the two embedding methods. In principle, as long as an embedding method can be converted to matrix factorization (Sec.~\ref{subsub:embedding_as_mf}), it can probably be incorporated in our study. We will discuss this later. %We briefly introduce the two methods below.

\textbf{DeepWalk}~\cite{perozzi2014deepwalk} first performs random walks on the network to sample a set of paths as a `corpus'. Each path in the corpus corresponds to a sentence, with each node as a word. Then a neural language model such as SkipGram~\cite{mikolov2013efficient} is applied on the paths to maximize the co-occurrence probability among the nodes appearing within a window $T$, which finally gives the network embedding.

\textbf{LINE}~\cite{tang2015line} learns network embedding by preserving the first-order (1st) and second-order (2nd) proximities. The 1st proximity is measured by the joint distribution between nodes $v_i$ and $v_j$ as:
\begin{equation}
p_1(v_i, v_j) = 1/(1+\exp(-\textbf{x}_{i}^{\top}\textbf{x}_j))
\end{equation}
The 2nd proximity is defined by the probability of context node $v_j$ being generated by node $v_i$:
\begin{equation}
p_2(v_j|v_i) = \exp(\textbf{x}_{j}^{\top}\textbf{x}_i)/(\sum\limits_k \exp(\textbf{x}_{k}^{\top}\textbf{x}_i))
\end{equation}
By minimizing the KL-divergence between the distributions above and the empirical distributions, the network embedding preserving the 1st and 2nd proximities, respectively, can be obtained.

\subsection{Embedding as Matrix Factorization}
\label{subsub:embedding_as_mf}

Previous work has proved that DeepWalk and LINE are implicitly solving a matrix factorization problem~\cite{qiu2018network}:
\begin{equation}\label{eq:matrixfac}
	\min_{X,Y} ||\hat{M}-XY^T||^2_F
\end{equation}
where $\hat{M}=\log(\max(M,1))$ is the matrix to factorize, depending on which network embedding method is used; $X$ is the node embedding matrix, $Y$ is the context embedding matrix learned together with $X$, and $||\cdot||^2_F$ denotes the squared Frobenious norm. For DeepWalk, the matrix $M$ is:
\begin{equation}\label{eq:deepwalk}
M=\log (vol(A)(\dfrac{1}{T} \sum_{r=1}^{T} (D^{-1}A)^r)D^{-1}) - \log b,
\end{equation}
and for LINE, the closed form of the matrix $M$ is:
\begin{equation}\label{eq:line}
M=\log (vol(A)(D^{-1}AD^{-1})) - \log b,
\end{equation}
where $vol(A)=\sum A_{ij}$ is the volume of network $A$, $D$ is the diagonal matrix with $D_{ii}$ representing the degree of node $v_i$, $T$ is the context window size, and $b$ is the number of negative sampling. Note that LINE is a special case of DeepWalk when $T=1$.

In particular, when seeing network embedding as matrix factorization, prior work has proven that the $K$-dimensional optimal embedding $X^*$'s loss $\mathcal{L} \left(X^*;A\right) = min_{X, Y} ||\hat{M}-XY^T||^2_F$ can be analytically computed (see \cite{bojchevski2019adversarial} for the details and the proof).

\begin{theorem}
	The loss of DeepWalk and LINE when using the optimal $K$-dimensional embedding $X^*$ for a given network $A$ is:
	\begin{equation}\label{equ:L2}
		%\mathcal{L} \left(X^*;A\right) = \sqrt{\sum_{p=K+1}^{|V|} \sigma_{p}^{2}},
		\mathcal{L} \left(X^*;A\right) = \left(\sum_{p=K+1}^{|V|} \sigma_{p}^{2}\right)^{\frac{1}{2}},
	\end{equation}
	where $\sigma_{p}$ is the $p$-th singular value of $\hat{M}$ with $\sigma_{1} \geq \sigma_{2} \cdots \geq \sigma_{|V|}$.
\end{theorem}

%From the perspective of matrix factorization, DeepWalk and LINE(2nd) are equivalent to optimizing $\min_{\hat{M}_K} ||\hat{M} - \hat{M}_K||^2_F$, where $\hat{M}_K$ is the best rank-$K$ approximation to $\hat{M}$.



%\subsection{Network Embeddings Utility Measurement}
%We obtain the privacy-preserving network embedding by manipulating the original network structure. However, the manipulations may change network embedding and result in data utility degeneration. In this section, we discuss how to measure the data utility of the network embedding when manipulating the network structure.
%
%For a given network $A$, the utility of the network embedding $X$ can be measured by the embedding quality loss $\mathcal{L} \left( A, X\right) $, and the optimal $X^*$ minimizes this loss:
%$$X^* = \min_X \mathcal{L} \left( A, X\right) $$
%Since the random walk based network embeddings are implicitly doing matrix factorization, we can quantify the loss by:
%
%\textbf{Theorem 1} \cite{bojchevski2019adversarial}. \textit{The loss of DeepWalk and LINE(2nd) when using the optimal embedding $X^*$ for a given network $A$ is: $\mathcal{L} \left( A, X^*\right) = {[\sum_{p=K+1}^{|V|} \sigma_{p}^{2}]}^{1/2}$, where $\sigma_{p}$ are the singular values of $\hat{M}$ sorted decreasingly $\sigma_{1} \geq \sigma_{2} \cdots \geq \sigma_{p}$, and $\hat{M}=\log(max(M, 1))$.
%}
%
%Given a manipulated network $A'$, assuming $X'$ is always the optimal network embedding learnt on $A'$, we can use Theorem 1 to quantify its embedding quality loss $\mathcal{L} (A', X')$. In order to control the utility loss of network embedding during manipulations, we set a utility loss budget $\Delta Q$ and restrict that $\mathcal{L} (A', X') \leq \Delta Q$.
%Given a manipulated network $A'$, we assume that $X'$ is always the optimal network embeddings learnt on $A'$. Then, the utility of network embedding $X'$ can be measured by $\mathcal{L} (A, X')$.


%\subsection{Privacy Leakage Computation}
%If the network embedding $X'$ is published, the attackers may correctly infer the existence of private links by launching a inference attack based on $X'$. In this section, we introduce the private link inference attack which we defend against, and define the privacy leakage of private links due to publishing $X'$.
%\begin{dfn}
%	\textbf{Private Link Inference Attack.} Given network embedding $X'$, the set of private node pairs $\mathscr{P}$, a private link inference attack is to classify the node pairs into positive node pairs that indicate existence of links and negative node pairs that mean absence of links by minimizing the expected inference loss:
%$$
%q ^* = \arg \min_q \mathbb{E}_{_{Y|X}} [Loss(Y,q)|X']
%$$
%where $Loss$ denotes the inference loss function, and $q^*$ is the optimal inference attack model by solving the private link inference attack problem.
%\end{dfn}

%As far as we know, most of link prediction algorithms predict the existence of links based on the similarity between nodes. Therefore, we use the similarity between private nodes to quantify the privacy leakage of private links. Specifically, We define the privacy leakage (PL) when publishing network embedding $X'$ as follows:
%$$PL(X')=Sims(X')_{\mathcal{P}_{pos}} - Sims(X')_{\mathcal{P}_{neg}}$$
%where the first item on the right represents the sum of similarities of positive node pairs, and the second item indicates the sum of similarities of negative node pairs. Larger $PL$ value means more privacy leakage of private links.

%$$PL=\sum_{ \left( i,j \right) \in \mathcal{P}_{pos} } \{ X'X'^T \}_{ij} - \sum_{ \left( i,j \right) \in \mathcal{P}_{neg} } \{ X'X'^T \}_{ij}$$
